Non-Autoregressive Predictive Coding for Learning Speech Representations from Local Dependencies

Self-supervised speech representations have been shown to be effective in a variety of speech applications. However, existing representation learning methods generally rely on the autoregressive model and/or observed global dependencies while generating the representation. In this work, we propose Non-Autoregressive Predictive Coding (NPC), a self-supervised method, to learn a speech representation in a non-autoregressive manner by relying only on local dependencies of speech. NPC has a conceptually simple objective and can be implemented easily with the introduced Masked Convolution Blocks. NPC offers a significant speedup for inference since it is parallelizable in time and has a fixed inference time for each time step regardless of the input sequence length. We discuss and verify the effectiveness of NPC by theoretically and empirically comparing it with other methods. We show that the NPC representation is comparable to other methods in speech experiments on phonetic and speaker classification while being more efficient.

==> figures/kernel_study.tex <==
\begin{figure}[t]
\centerline{\includegraphics[width=7cm]{kernel_study.jpeg}}
\vspace{-7pt}
\caption{\small \alex{2 Layer, $M_\text{in}=5$, ser not finalized}}
\vspace{-10pt}
\label{fig:kernel}
\end{figure}

==> figures/mask_study.tex <==
\begin{figure}[t]
\centerline{\includegraphics[width=7cm]{mask_study.jpeg}}
\caption{\small \alex{2 Layer, $R=23$, ser not finalized}}
\vspace{-10pt}
\label{fig:mask}
\end{figure}

==> tables/ablation.tex <==
\begin{table}[t]
\small
\centering
\begin{threeparttable}

\caption{\small Mean Opinion Score (MOS) ratings with 95\% confidence intervals for naturalness.}

\begin{tabular}{ l| c| c c}
\toprule
\multicolumn{1}{l|}{Method}  & PER   & Spkr.ER  \\ \hline
 3-Layerd ConvBlock.        &   27.7     &      \\\hline
 AE bottlenock              &       &      \\ 
 No VQ.                     &       &      \\ \hline
 2 Layered Network & 28.8 & \\
 Masked ConvBlock at last layer only & 29.7     &      \\ 
 

\bottomrule
\end{tabular}
\vspace{-2pt}
%\vspace{-7pt}
\label{table:mos}
\end{threeparttable}
\end{table}


==> tables/per_result.tex <==
\begin{table}[t]
\small
\centering
\begin{threeparttable}

\caption{\small Phoneme error rate (\%) on different amount of paired data.}

\begin{tabular}{l| c| c| c| c}
\toprule
\multicolumn{1}{l|}{Method}  & 20 min & 15 min & 10 min & 5 min\\ \hline 
Baseline          & 29.4 & 33.2 & 41.2 & 55.7\\    
Ren et al.~\cite{ren2019almost}\textsuperscript{\textdagger} & 11.7 & -    & 64.2 & -   \\ \hline \hline   
Ours & & & & \\ \hline
- w/o codebook & 29.9 & 33.2 & 41.4 & 56.2  \\ 
- w/~ codebook  & 25.5 & 29.0 & 35.2 & 49.3 \\

\bottomrule
\end{tabular}
\vspace{-2pt}
\begin{tablenotes}
\item{\textdagger} \small{\text{Used unpaired text besides unpaired speech.}}
\end{tablenotes}
\vspace{-7pt}
\label{table:per}
\end{threeparttable}
\end{table}

